Supervised Contrastive Learning for Snapshot Spectral Imaging Face Anti-Spoofing

This study reveals a cutting-edge re-balanced contrastive learning strategy aimed at strengthening face anti-spoofing capabilities within facial recognition systems, with a focus on countering the challenges posed by printed photos, and highly realistic silicone or latex masks. Leveraging the HySpeFAS dataset, which benefits from Snapshot Spectral Imaging technology to provide hyperspectral images, our approach harmonizes class-level contrastive learning with data resampling and an innovative real-face oriented reweighting technique. This method effectively mitigates dataset imbalances and reduces identity-related biases. Notably, our strategy achieved an unprecedented 0.0000\% Average Classification Error Rate (ACER) on the HySpeFAS dataset, ranking first at the Chalearn Snapshot Spectral Imaging Face Anti-spoofing Challenge on CVPR 2024.

==> Sections/Figures/motivation.tex <==
\begin{figure}[htp]
\begin{center}
\includegraphics[width=0.9\linewidth]{./Figures/}
\end{center}
\caption{Motivation}
\label{fig:motivation} 
\end{figure}

==> Sections/Tables/ablation.tex <==
\begin{table*}[!htp]
  \centering
  \caption{Ablation studies of of XXX.} 
   \resizebox{1\columnwidth}{!} {
  %\fontsize{8}{8}\selectfont
  \begin{tabular}{l|ccccccc}
\toprule 
Method1& &&&&&\\
Method2& &&&&&\\
Method3& &&&&&\\
Method4& &&&&&\\
\bottomrule
\end{tabular}
}
  \label{tab:ablation}
\end{table*}


==> Sections/Tables/metric_score.tex <==
\begin{table*}[!htp]
  \centering
  \caption{Quantitative metric comparison of XXX.} 
   \resizebox{1\columnwidth}{!} {
  %\fontsize{8}{8}\selectfont
  \begin{tabular}{l|ccccccc}
\toprule 
Method1& &&&&&\\
Method2& &&&&&\\
Method3& &&&&&\\
Method4& &&&&&\\
\bottomrule
\end{tabular}
}
  \label{tab:metric_score}
\end{table*}

